Execution Templates: Caching Control Plane Decisions for Strong Scaling of Data Analytics

Control planes of cloud frameworks trade off between scheduling granularity and performance. Centralized systems schedule at task granularity, but only schedule a few thousand tasks per second. Distributed systems schedule hundreds of thousands of tasks per second but changing the schedule is costly. We present execution templates, a control plane abstraction that can schedule hundreds of thousands of tasks per second while supporting fine-grained, per-task scheduling decisions. Execution templates leverage a program's repetitive control flow to cache blocks of frequently-executed tasks. Executing a task in a template requires sending a single message. Large-scale scheduling changes install new templates, while small changes apply edits to existing templates. Evaluations of execution templates in Nimbus, a data analytics framework, find that they provide the fine-grained scheduling flexibility of centralized control planes while matching the strong scaling of distributed ones. Execution templates support complex, real-world applications, such as a fluid simulation with a triply nested loop and data dependent branches.

==> discussion.tex <==
\section{Discussion}
\label{sec:discuss}

Execution templates are a general abstraction that can be applied to many
frameworks.  However, the characteristics laid out in
Section~\ref{sec:design} can be simpler to incorporate in some systems
than others. Here, we consider two major data analytics frameworks
Spark~\cite{spark} and Naiad~\cite{naiad} for possibly adopting the execution
templates design. We hope that that this discussion motivates rethinking the
design decisions in future frameworks.

\medskip\noindent\textbf{Templates in Spark:}
Incorporating execution templates into Spark would require three significant
changes to its data model and execution model.  First, workers would require
queuing tasks and resolving dependencies locally. This does not align with the
existing lazy evaluation model where controller is exclusively responsible for
ordering the tasks.  Adding execution templates would require adding dependency
metadata to tasks as well as worker control logic.  Second, Spark workers need
to be able to exchange data directly. Otherwise, every access of a new data
object in global operations (e.g. shuffles) requires a lookup at the controller.
Last, efficient implementation of execution templates beyond basic blocks with
single stage requires caching data identifiers for reuse. Current immutable data
model requires explicit data assignment by controller. A mutable data model
could solve this problem.


\medskip\noindent\textbf{Templates in Naiad:}
Naiad execution model is an extreme case of templates without flexibility of
execution templates. Controller template is generated at the compile time as the
"logical graph", and worker templates are installed at the beginning of the
iterative dataflow computation by mapping logical graph to physical graphs on
each worker node. Since the message and notification deliveries in current
distributed design depends on the rigid mappings, task migrations or changes in
the mappings are impossible once the computation starts. One suggestion is to
add support for dynamic edits at the task granularity to the physical graph
installed on each worker. This would allow Naiad to spawn task at task
granularity as opposed to the entire iterative computation.  Question remains on
how the new changes affect the performance of Naiad's distributed progress
tracking protocol.


